Properties of a Projected Network of a Bipartite Network

Bipartite Graph is often a realistic model of complex networks where two different sets of entities are involved and relationship exist only two entities belonging to two different sets. Examples include the user-item relationship of a recommender system, actor-movie relationship of an online movie database systems. One way to compress a bipartite graph is to take unweighted or weighted one mode projection of one side vertices. Properties of this projected network are extremely important in many practical situations (say the selection process of influencing nodes for viral marketing). In this paper, we have studied the topological properties for projected network and some theoretical results are proved including the presence of cliques, connectedness for unweighted projection and maximum edge weight for weighted projected network.

==> refer <==

@article{Atzori10,
  title                    = {{The Internet of Things: A survey}},
  author                   = {Luigi Atzori and Antonio Iera and Giacomo Morabito},
  journal                  = {Computer Networks (Elsevier)},
  year                     = {2010},
  number                   = {15},
  pages                    = {2787--2805},
  volume                   = {54}
}

@book{bondy1976graph,
  title={Graph theory with applications},
  author={Bondy, John Adrian and Murty, Uppaluri Siva Ramachandra},
  volume={290},
  year={1976},
  publisher={Citeseer}
}

@article{zweig2011systematic,
  title={A systematic approach to the one-mode projection of bipartite graphs},
  author={Zweig, Katharina Anna and Kaufmann, Michael},
  journal={Social Network Analysis and Mining},
  volume={1},
  number={3},
  pages={187--218},
  year={2011},
  publisher={Springer}
}

@article{vazquez2002modeling,
  title={Modeling of protein interaction networks},
  author={V{\'a}zquez, Alexei and Flammini, Alessandro and Maritan, Amos and Vespignani, Alessandro},
  journal={Complexus},
  volume={1},
  number={1},
  pages={38--44},
  year={2002},
  publisher={Karger Publishers}
}

@article{ravasz2002hierarchical,
  title={Hierarchical organization of modularity in metabolic networks},
  author={Ravasz, Erzs{\'e}bet and Somera, Anna Lisa and Mongru, Dale A and Oltvai, Zolt{\'a}n N and Barab{\'a}si, A-L},
  journal={science},
  volume={297},
  number={5586},
  pages={1551--1555},
  year={2002},
  publisher={American Association for the Advancement of Science}
}

@article{ozgur2008identifying,
  title={Identifying gene-disease associations using centrality on a literature mined gene-interaction network},
  author={{\"O}zg{\"u}r, Arzucan and Vu, Thuy and Erkan, G{\"u}ne{\c{s}} and Radev, Dragomir R},
  journal={Bioinformatics},
  volume={24},
  number={13},
  pages={i277--i285},
  year={2008},
  publisher={Oxford Univ Press}
}

@article{zhou2007bipartite,
  title={Bipartite network projection and personal recommendation},
  author={Zhou, Tao and Ren, Jie and Medo, Mat{\'u}{\v{s}} and Zhang, Yi-Cheng},
  journal={Physical Review E},
  volume={76},
  number={4},
  pages={046115},
  year={2007},
  publisher={APS}
}

@book{diestel2000graph,
  title={Graph theory $\{$graduate texts in mathematics; 173$\}$},
  author={Diestel, Reinhard},
  year={2000},
  publisher={Springer-Verlag Berlin and Heidelberg GmbH \& amp}
}

@inproceedings{matsuo2009community,
  title={Community gravity: measuring bidirectional effects by trust and rating on online social networks},
  author={Matsuo, Yutaka and Yamamoto, Hikaru},
  booktitle={Proceedings of the 18th international conference on World wide web},
  pages={751--760},
  year={2009},
  organization={ACM}
}

@article{huang2007analyzing,
  title={Analyzing consumer-product graphs: Empirical findings and applications in recommender systems},
  author={Huang, Zan and Zeng, Daniel D and Chen, Hsinchun},
  journal={Management science},
  volume={53},
  number={7},
  pages={1146--1164},
  year={2007},
  publisher={INFORMS}
}

@inproceedings{lattanzi2009affiliation,
  title={Affiliation networks},
  author={Lattanzi, Silvio and Sivakumar, D},
  booktitle={Proceedings of the forty-first annual ACM symposium on Theory of computing},
  pages={427--434},
  year={2009},
  organization={ACM}
}

@book{ricci2011introduction,
  title={Introduction to recommender systems handbook},
  author={Ricci, Francesco and Rokach, Lior and Shapira, Bracha},
  year={2011},
  publisher={Springer}
}

@inproceedings{shang2008personal,
  title={Personal Recommendation using Weighted Bipartite Graph Projection},
  author={Shang, Ming-Sheng and Fu, Yan and Chen, Duan-Bin},
  booktitle={Apperceiving Computing and Intelligence Analysis, 2008. ICACIA 2008. International Conference on},
  pages={198--202},
  year={2008},
  organization={IEEE}
}

@article{gustafsson2014describing,
  title={Describing citation structures in sport burnout literature: A citation network analysis},
  author={Gustafsson, Henrik and Hancock, David J and C{\^o}t{\'e}, Jean},
  journal={Psychology of Sport and Exercise},
  volume={15},
  number={6},
  pages={620--626},
  year={2014},
  publisher={Elsevier}
}

@book{cormen2009introduction,
  title={Introduction to algorithms},
  author={Cormen, Thomas H},
  year={2009},
  publisher={MIT press}
}


@book{bollobas2013modern,
  title={Modern graph theory},
  author={Bollob{\'a}s, B{\'e}la},
  volume={184},
  year={2013},
  publisher={Springer Science \& Business Media}
}

@inproceedings{li2013link,
  title={Link recommendation for promoting information diffusion in social networks},
  author={Li, Dong and Xu, Zhiming and Li, Sheng and Sun, Xin and Gupta, Anika and Sycara, Katia},
  booktitle={Proceedings of the 22nd International Conference on World Wide Web},
  pages={185--186},
  year={2013},
  organization={ACM}
}

@article{an2016diffusion,
  title={Diffusion-like recommendation with enhanced similarity of objects},
  author={An, Ya-Hui and Dong, Qiang and Sun, Chong-Jing and Nie, Da-Cheng and Fu, Yan},
  journal={Physica A: Statistical Mechanics and its Applications},
  year={2016},
  publisher={Elsevier},
  pages                    = {708--715},
  volume                   = {461}
}

@inproceedings{bakshy2012role,
  title={The role of social networks in information diffusion},
  author={Bakshy, Eytan and Rosenn, Itamar and Marlow, Cameron and Adamic, Lada},
  booktitle={Proceedings of the 21st international conference on World Wide Web},
  pages={519--528},
  year={2012},
  organization={ACM}
}

@article{guille2013information,
  title={Information diffusion in online social networks: A survey},
  author={Guille, Adrien and Hacid, Hakim and Favre, Cecile and Zighed, Djamel A},
  journal={ACM SIGMOD Record},
  volume={42},
  number={2},
  pages={17--28},
  year={2013},
  publisher={ACM}
}

@article{abiad2013algebraic,
  title={Algebraic characterizations of regularity properties in bipartite graphs},
  author={Abiad, Aida and Dalf{\'o}, Cristina and Fiol, Miquel {\`A}ngel},
  journal={European Journal of Combinatorics},
  volume={34},
  number={8},
  pages={1223--1231},
  year={2013},
  publisher={Elsevier}
}

